Bias in, Bias out: Annotation Bias in Multilingual Large Language Models

Annotation bias in NLP datasets remains a major challenge for developing multilingual Large Language Models (LLMs), particularly in culturally diverse settings. Bias from task framing, annotator subjectivity, and cultural mismatches can distort model outputs and exacerbate social harms. We propose a comprehensive framework for understanding annotation bias, distinguishing among instruction bias, annotator bias, and contextual and cultural bias. We review detection methods (including inter-annotator agreement, model disagreement, and metadata analysis) and highlight emerging techniques such as multilingual model divergence and cultural inference. We further outline proactive and reactive mitigation strategies, including diverse annotator recruitment, iterative guideline refinement, and post-hoc model adjustments. Our contributions include: (1) a typology of annotation bias; (2) a synthesis of detection metrics; (3) an ensemble-based bias mitigation approach adapted for multilingual settings, and (4) an ethical analysis of annotation processes. Together, these insights aim to inform more equitable and culturally grounded annotation pipelines for LLMs.

==> table/bias_table.tex <==
\vspace{1em}
\begin{table*}[h]
\centering
\caption{Summary of annotation bias types in NLP}
\label{tab:bias-summary}
\begin{tabular}{|p{3cm}|p{5cm}|p{7cm}|}
\hline
\textbf{Bias Type} & \textbf{Source/Mechanism} & \textbf{Examples and Challenges} \\ \hline
\textbf{Instruction Bias} & Task framing: guidelines, prompts, and interfaces carrying implicit assumptions & Narrow sentiment labels ignoring irony~\cite{Mohammad:Emotion:2016}; culturally unaware toxicity definitions~\cite{Sap:ACL:2019}; unvalidated few-shot prompts~\cite{Schick:TACL:2022} \\ \hline
\textbf{Annotator Bias} & Annotators’ demographics, beliefs, experiences, and subjective interpretations & Global North crowdworkers labelling data from Global South~\cite{Bender:ACM:2021}; majority voting ignoring disagreement~\cite{Aroyo:IEEE:2015} \\ \hline
\textbf{Contextual and Cultural Bias} & Broader sociocultural and linguistic norms embedded in data collection and interpretation & Labels not translating across cultures~\cite{Ponti:EMNLP:2020:xcopa}; multimodal signals misinterpreted across cultures~\cite{Lisa:PSPI:2019} \\ \hline
\end{tabular}
\end{table*}
